PEERNet: An End-to-End Profiling Tool for Real-Time Networked Robotic Systems

Networked robotic systems balance compute, power, and latency constraints in applications such as self-driving vehicles, drone swarms, and teleoperated surgery. A core problem in this domain is deciding when to offload a computationally expensive task to the cloud, a remote server, at the cost of communication latency. Task offloading algorithms often rely on precise knowledge of system-specific performance metrics, such as sensor data rates, network bandwidth, and machine learning model latency. While these metrics can be modeled during system design, uncertainties in connection quality, server load, and hardware conditions introduce real-time performance variations, hindering overall performance. We introduce PEERNet, an end-to-end and real-time profiling tool for cloud robotics. PEERNet enables performance monitoring on heterogeneous hardware through targeted yet adaptive profiling of system components such as sensors, networks, deep-learning pipelines, and devices. We showcase PEERNet's capabilities through networked robotics tasks, such as image-based teleoperation of a Franka Emika Panda arm and querying vision language models using an Nvidia Jetson Orin. PEERNet reveals non-intuitive behavior in robotic systems, such as asymmetric network transmission and bimodal language model output. Our evaluation underscores the effectiveness and importance of benchmarking in networked robotics, demonstrating PEERNet's adaptability. Our code is open-source and available at github.com/UTAustin-SwarmLab/PEERNet.

==> sections/experiments.tex <==
We validate \name by implementing and profiling three edge and cloud robotic systems. We demonstrate that \name is modular and robust, capable of precise profiling of diverse systems. All of our experiments are conducted on physical hardware and live wireless networks. Our first experiment, offloaded image classification, demonstrates our profiler's ability to generalize to common cloud robotics systems. Our second experiment demonstrates \name's identification and profiling of complex behavior in LLM inference. Finally, our third experiment, a teleoperation example on a Franka Emika Panda robot arm, demonstrates \name's ability to profile arbitrary systems in a modular fashion.

\input{figure_latex/efficientnet-paired}
\input{figure_latex/llava}

\subsection{Offloaded Image Classification with EfficientNetV2}
Consider a self-driving car performing image classification in real-time on a video stream. For such a resource-constrained edge device, offloading image classification to cloud servers over wireless networks is a viable solution. Suppose further that our self-driving car has access to a bank of image classification models, each with varying model complexities. For one to develop methods to intelligently select which image classifier from the bank to run, data on the inference latency of each model running locally and on cloud servers are essential. 

We implement such an offloaded image classification system with the following parameters. The edge device is an Nvidia Jetson AGX Orin 64Gb, a popular single-board computer for ML on the edge. The bank of models is the EfficientNetV2 family of image classifiers \cite{tan2021efficientnetv2}, trained on the ImageNet \cite{deng2009imagenet} dataset, which includes three model variants: small, medium, and large. A remote server with an Nvidia A5000 GPU plays the role of a cloud server. The remote server is configured as an NTP server, with the Nvidia Jetson configured as an NTP client. 
As this is a case of offloaded computation, the experiment is fully specified through \name's CLI for offloaded inference. We specify a network type, provide domain names and IP addresses for each device, and specify a model to be run, either locally or in the cloud. Appendix B contains the precise terminal commands issued to reproduce our offloaded image classification experiment.

Figure \ref{fig:efficientnet-paired} displays the performance of each variant of EfficientNetV2 when run locally and on a cloud server. \name's profiling enables us to precisely quantify the latency of each variant of EfficientNetV2 locally and on the cloud server. We see that each variant running locally is roughly 2.5 times slower than the same model running in the cloud. A more subtle observation from the profiling is the high variance in inference latency in the cloud compared to the low variance in inference latency locally. This observation is consistent with the fact that cloud servers have many users, while edge devices rarely run many parallel processes. Thus, the variance in inference latency in the cloud is large compared to the variance in latency on the edge.
In summary, this experiment demonstrates the powerful abstraction of offloaded computation as a framework to benchmark in and validates \name's CLI as a modular and easy-to-use method to obtain precise profiling data on offloaded computation systems.

\input{figure_latex/table}

\subsection{LLM Inference at the Edge}
Recently, the robotics community has begun to adopt LLMs in robotic pipelines. These models provide reasoning and planning capabilities, performing roles such as task-planning \cite{sharan2024plan, vemprala2023chatgpt}. Furthermore, multi-modal LLMs such as LLaVA \cite{liu2024visual} are particularly suited to robotics applications due to the ability to reason about images and video. Due to the size of modern LLMs, many applications adopt a cloud inference model, where LLMs are served over wireless networks. However, with advancing edge hardware and powerful GPUs at the edge, the feasibility of LLM inference at the edge is an open question.

In this experiment, we use \name to profile the performance of LLaVA \cite{liu2024visual}, a multi-modal LLM capable of image reasoning on edge inference. We implement and benchmark the edge-inference system using \name's utilities, and demonstrate the ability to obtain complex information about model performance.

In our experimental setup, the edge device is an Nvidia Jetson AGX Orin 64Gb. The multi-modal LLM we use is LLaVA-v1.5-7b\cite{liu2023improved}. We focus our profiling on understanding the output length of LLM responses and the relationship between output length and inference latency.

Figure \ref{fig:llava} presents collected data on the performance of LLM inference at the edge, along with a test prompt and image, from the Waymo Open Dataset \cite{Sun_2020_CVPR}. Benchmarking with \name reveals that for a particular image and prompt, LLaVA-v1.5's output length is strongly bimodal. Furthermore, we note that our edge device can produce between 8 and 15 tokens per second, corresponding to between 5 and 20 seconds per inference with a particular prompt. 

\subsection{Teleoperation of a Robotic Arm}

Teleoperation, in which a physical robot is controlled remotely by another machine or human, is a prevalent use case of cloud robotics, with implementations in self-driving \cite{tener2022driving, zhang2020toward}, augmented reality \cite{walker2019robot}, and telesurgery \cite{sedaghat2021rt, barba2022remote}. We design, implement, and benchmark a teleoperation system for a Franka Emika Panda robot arm to demonstrate the flexibility of \name.

\input{figure_latex/franka-stacked-barplot}

We implement and profile a teleoperation pipeline accomplishing a vision-based robot manipulation task. In this task, the manipulator must start from its initial configuration $50$cm above the table and precisely reach a blue square with image observations from two camera angles. We employ a CNN-based control policy trained with visual reinforcement learning to ensure consistency in task performance \cite{zhao2023learning}. The robot arm is controlled by an Nvidia Jetson AGX Orin 64Gb (single-board computer), which is wirelessly connected to a desktop machine with an Nvidia 3090 graphics card for teleoperation. 
We implement three forms of the teleoperation experiments: \textit{Local}, \textit{Cloud-Uncompressed}, and \textit{Cloud-Compressed}. 
\begin{enumerate}
    \item In the \textit{Local} form, the Nvidia Jetson collects image observations, performs inference using the CNN controller, and sends actions to the robot arm through a ROS network. 
    
    \item In the \textit{Cloud-Uncompressed} form, the Nvidia Jetson offloads full-resolution images to the desktop machine over a WiFi network. The desktop machine performs inference using the same CNN controller and transmits actions back to the Nvidia Jetson, which forwards actions to the robot arm through the ROS network. 

    \item In the \textit{Cloud-Compressed} form, the Nvidia Jetson collects image observations, downsamples them to lower the resolution, and offloads downsampled images to the desktop machine. The desktop machine performs inference and transmits actions back to the Nvidia Jetson.
\end{enumerate}

The desktop machine is configured as an NTP server, with the edge device as an NTP client, to sync the time between devices. We use Chrony for the NTP server/client implementation. During the experiment, the edge device and cloud device communicate through the \name Network module's TCP implementation, which allows one-way delay timing given synced clocks. Utilities from \name's logging module are used to profile the performance of the CNN controller.

Figure \ref{fig:franka-stacked-barplot} shows the relative latency of teleoperated control between the three forms of teleoperation. Although local inference is slower than inference in the cloud, communication costs outweigh the differences in inference latency when uploading full-resolution images. However, for downsampled images, the network is sufficiently fast to realize the benefit of inference in the cloud. Thus, compressing and offloading results in minimal end-to-end latency, of $17.67$ ms on average. We also note the asymmetry in networking--- as the uploaded images are much larger than the downloaded actions, the vast majority of network latency is attributed to upload. This serves as an example for how \name provides detailed profiling information on specific systems with specific, real hardware.





==> sections/introduction_1.tex <==
% \begin{itemize}
%     \item Questions/Content Feedback
%     \begin{itemize}
%         \item Include some form of scenarios, a few, to make the point very clear. 
%         \item Given that my teleoperation system needs end to end control of 50 ms, I have a wifi network, and a jetson device at the edge, what should I provision the cloud to be?
%         \item I have a nvidia jetson at the edge (budget constraint), a trusted wifi network, and AV, what model should I run locally (eg efficient net small, large, etc).
%         \item Conversley, I have any model I want locally, but now there is 5G, how much better is my inference?
%         \item 6G is not even out there, but this stack can be used in future networkk that have yet to be designed
%         \item To the "average" reader, this may seem like just a profiling and benchmarking tool, however it is much more sophisticated and nuanced. First we see that Wireless networks are designed high assymetrically, and our tool can provide insight on highly non-intuituve information to the users. 
%         \begin{itemize}
%             \item eg: I might tell you that it is better to teleoperate the system with highly compressed data, opposed to using a really small network locally without the marginal accuacy 
%         \end{itemize}
%         \item Include more user questions?
%     \end{itemize}
% \end{itemize}




Edge and cloud robotic systems \cite{kehoe2015survey, mao2017survey} have emerged as resilient solutions for tackling compute, power, and latency constraints in robotics.
These systems find applications across diverse domains such as self-driving vehicles \cite{kumar2012cloud} and teleoperated robotic surgery \cite{berkelman2009compact}, showcasing their versatility and effectiveness.
However, optimizing these systems necessitates real-time measurement and monitoring of system-specific performance metrics such as data rates, network bandwidth, and machine learning model latency. 
Consider, for example, a teleoperated autonomous vehicle. This system will have multi sensor data including lidar and video feed transmitted over high traffic networks to a cloud device running a inference model to teleoperate this vehicle. Given an asymmetric wifi network with \textcolor{blue}{250} Mbps download and \textcolor{blue}{50} Mbps upload speeds, and a Nvidia Jetson Orin 64Gb device as the cloud running inference, what image classification model should be provisioned on the Jetson to enable highest decision accuracy while maintaining maximum end to end latency of 200 ms for safe operation? Conversely, we now introduce a 5G network, how will the network latency and inference accuracy be affected? If the vehicle is in network constrained environments and needs to perform inference locally, which model should be deployed on the edge to give the best inference results while bypassing network latency and given the local compute constraints? In such scenarios, understanding and ensuring the reliability of sensors and networks becomes paramount. 
Thus, access to real-time system-specific performance metrics is essential for tracking end-to-end latency and ensuring the reliability of robotic systems.

\par Conventional methods for accessing system-specific performance metrics in cloud and edge robotic systems fall into two categories: isolated benchmarks and end-to-end system benchmarks. 
Generally, isolated benchmarks for cloud and edge robotics focus on profiling individual components such as sensors or Machine Learning (ML) models. Although easy to implement and generalizable to a wide array of real hardware, these methods fail to reflect the complex interdependencies between components in edge and cloud robotic systems \pohan{such as?}. \pohan{mention your one-way profiling advantage.}
On the contrary, existing end-to-end system benchmarks \pohan{citations} profile components in-loop on fully built systems, but often ignore networking as a significant component of robotic systems and generally fail to put forward a comprehensive software platform for modular profiling.

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{figures/figure-1.pdf}
    \caption{\textcolor{blue}{New name} is an end-to-end profiling tool for cloud robotics. \textcolor{blue}{New name} is modular, allowing users to specify custom configurations of sensors, networks, and devices in a benchmark configuration, and inject custom external modules. Detailed profiles, complete with asymmetric network timing, are generated.}
    \label{fig:system-overview}
\end{figure}

\par For these reasons, we propose \textcolor{blue}{New Name}, a novel end-to-end profiling tool built for networked cloud and edge robotics. 
By modeling arbitrary cloud robotic systems as combinations of sensors, networks, and computation, \textcolor{blue}{New Name} is better suited to profile cloud and edge robotics, as it is capable of detailed profiling of arbitrary user-defined systems. As shown in Figure \ref{fig:system-overview}, \textcolor{blue}{New Name} emphasizes end-to-end benchmarking by profiling the entire flow of data, allowing us to profile at a level of detail not possible with isolated benchmarks.



\par For these reasons, we propose \textcolor{blue}{New Name}, a novel end-to-end profiling tool built with networked cloud and edge robotics in mind. By modeling arbitrary cloud robotic systems as combinations of sensors, networks, and computation, our method is better suited to profiling cloud and edge robotics as it is capable of detailed profiling of arbitrary, user-defined systems. This is the first tool which integrates with off the shelf devices and products such as Nvidia Jetsons, Google Edge TPU, and Robot Operating System (ROS) that allows the user to systematically benchmark any aspects which contribute to the operation of a successful cloud and edge robotics system.


As shown in Figure \ref{fig:system-overview}, our system emphasizes end-to-end benchmarking by profiling over the entire flow of data, allowing us to profile at a level of detail not possible with isolated benchmarks.

% Although \textcolor{blue}{New Name} may seem like a simple benchmarking and profiling tool, it actually provides highly sophisticated and nuanced capabilities which can provide insight on highly non-intuitive information to the users to design and utilize highly capable systems.

\par In summary, our contributions are:

\begin{enumerate}
    \item \textbf{Introduction of the first end-to-end benchmarking tool for cloud robotics:} We introduce \textcolor{blue}{newName}, a comprehensive framework and Python package tailored to end-to-end benchmarking of custom networked-robotics scenarios. \textcolor{blue}{NewName} considers networks to be significant in robotic systems, profiles across the entire flow of data, and allows benchmarking custom robotic systems.
    
    \item \textbf{Enhanced Modularity and Accessibility:} \textcolor{blue}{NewName} boasts a high degree of modularity and accessibility, facilitated by highly modular implementation and a comprehensive Command-Line Interface (CLI) which allows users to define custom cloud robotics setups to profile, even allowing users to pass external programs into the benchmarking framework.

    \item \textbf{Attention to Asymmetric Networks:} \textcolor{blue}{NewName} implements a custom scheme for timing one-way network transmission with synced device clocks. This form of profiling is more specific than common round-trip delay estimation, offering greater specificity in collected data, particularly in cloud robotics systems with ``asymmetric" networks, where devices often upload much more data than they download.
   
    \item \textbf{Exploration of Robotics Scenarios:} Through rigorous experimentation, we explore three distinct robotics scenarios encompassing offloaded inference and teleoperated robotics. Leveraging the capabilities of \textcolor{blue}{newName}, we conduct comprehensive benchmarking to assess performance across varied implementations of networked robotics. Our findings underscore the end-to-end benchmarking capabilities of our framework, emphasizing its prowess in profiling, extensibility, and modularity.
\end{enumerate}


% \par Common approaches to the data acquisition problem of profiling cloud and edge robotic systems fall into two categories: isolated benchmarks and end-to-end system benchmarks. Generally, isolated benchmarks for cloud and edge robotics focus on profiling individual components such as sensors or Machine Learning (ML) models. While easy to implement and generalizable to a wide array of real hardware, these approaches fail to reflect the complex interdependencies between components in cloud and edge robotic systems. Existing works in end-to-end system benchmarking profile components in-loop on fully built systems, but often ignore networking as a significant component of robotic systems, and generally fail to put forward a comprehensive software platform for modular profiling. Today, as a result, we have no way of profiling these systems for bottlenecks in latency \textcolor{blue}{and so forth}. 
